From Reality to Recognition: Evaluating Visualization Analogies for Novice Chart Comprehension

Novice learners often have difficulty learning new visualization types because they tend to interpret novel visualizations through the mental models of simpler charts they have previously encountered. Traditional visualization teaching methods, which usually rely on directly translating conceptual aspects of data into concrete data visualizations, often fail to attend to the needs of novice learners navigating this tension. To address this, we conducted an empirical exploration of how analogies can be used to help novices with chart comprehension. We introduced visualization analogies: visualizations that map data structures to real-world contexts to facilitate an intuitive understanding of novel chart types. We evaluated this pedagogical technique using a within-subject study (N=128) where we taught 8 chart types using visualization analogies. Our findings show that visualization analogies improve visual analysis skills and help learners transfer their understanding to actual charts. They effectively introduce visual embellishments, cater to diverse learning preferences, and are preferred by novice learners over traditional chart visualizations. This study offers empirical insights and open-source tools to advance visualization education through analogical reasoning.

==> Sections/result_reduced.tex <==
In this results section, we explore the effectiveness of visualization analogies across 5 dimensions. First, we evaluate how these analogies impact performance and cognitive load in visual analytic tasks compared to standard charts \textbf{[RQ1]}. Subsequently, we investigate their role as a teaching tool by exploring the learning transfer effects from analogy charts to standard charts \textbf{[RQ2]}. We also address potential trade-offs to determine whether visual embellishments in analogies influence users' attention and interpretation accuracy \textbf{[RQ3]}. Furthermore, we assess the generalizability of visualization analogies across diverse VARK learning preferences \textbf{[RQ4]}. Finally, we capture learners' perceptions and analyze their engagement and comprehension preferences regarding these visualization methods \textbf{[RQ5]}.

\subsection{RQ1 [Performance \& Load]: Effectiveness of Visualization Analogies}

\textbf{Visualization analogies significantly enhance users' performance in visual analytic tasks compared to standard charts.} Participants who used visualization analogies achieved higher performance scores (\textit{M = 22.91, SD = 7.30}) than those who used standard charts (\textit{M = 19.77, SD = 6.65}). A paired t-test revealed a statistically significant difference (\textit{p = .0004}). This result indicates strong evidence that visualization analogies enhance performance compared to standard charts.

\begin{figure}[htb]
  \centering
  \includegraphics[width=1\linewidth]{Figures/RQ1.png}
  \caption{\label{fig:rq1result}
           An overview of visual analytic tasks result grouped by chart type (from left to right): the performance score on each technique, time spend on each technique.}
\end{figure}

We observed that specific charts are inherently easier or harder to interpret. We performed a cluster analysis on the performance scores to categorize the charts based on difficulty levels. The optimal clustering resulted in two groups, allowing us to separate the charts into \textbf{simple} and \textbf{complex} categories.

\textbf{Analogy charts show varying levels of effectiveness depending on chart complexity, particularly excelling with simpler charts.} For simple charts, participants using analogy charts had a average performance score of \textit{27.81 (SD = 4.66)}, compared to \textit{23.83 (SD = 4.54)} for standard charts. This difference was highly significant (\textit{p < .0001}). For complex charts, the analogy condition yielded a average score of \textit{19.96 (SD = 7.03)}, while the standard condition had a average of \textit{17.33 (SD = 6.54)}. This was also a significant difference (\textit{p = .015}). These results show that visualization analogies enhance performance across chart difficulties, with the most pronounced effect seen in easier charts.

Our mixed-effects model further confirmed these findings. The fixed factors included visualization technique, chart difficulty, average time spend, and order of exposure. The model revealed that analogy charts resulted in an average of \textit{11\%} higher performance scores than standard charts. Difficulty level was also highly significant, simpler charts had \textit{19\%} higher performance scores than complex charts on average. Notably, the average time spent on tasks was not a significant factor, indicating that participants could understand analogy charts quickly and still demonstrate a high level of comprehension.

\begin{figure}[htb]
  \centering
  \includegraphics[width=1\linewidth]{Figures/RQ2.png}
  \caption{\label{fig:rq2}
            Self-reported evaluations result (from left to right): Each plot displays cognitive load dimensions (mental demand, effort, and frustration) of NASA-TLX, first-exposure perceptions of understanding, ease of interpretation, and confidence.}
\end{figure}

Looking at the self-reported dimensions (Figure~\ref{fig:rq2}), \textbf{Visualization analogies led to significantly higher comprehension and confidence compared to standard charts.} Participants felt they understood the charts better when first exposed to analogy charts. Comprehension ratings were significantly higher \textit{(p = 0.001)}. Confidence ratings were also significantly higher for analogy charts than standard charts \textit{(p = 0.016)}. On the downside, the ease of interpretation did not reach statistical significance \textit{(p = 0.086)}. This suggests that both methods maintain a certain level of cognitive friction necessary for extracting insights. 

To further explore the overall load introduced by analogies, we examined how different dimensions of cognitive load were impacted. \textbf{Visualization analogies reduce cognitive load in relevant dimensions.} Participants experienced lower mental demand when using analogy charts \textit{(p = 0.002)}. They reported less effort \textit{(p = 0.010)} and less frustration \textit{(p < 0.001)} with analogy charts compared to standard charts. These findings suggest that visualization analogies improve performance and make tasks less cognitively demanding.


\subsection{RQ2 [Learning Transfer]: Enhancing Comprehension from Analogy to Standard Charts}

\begin{figure}[htb]
  \centering
  \includegraphics[width=1\linewidth]{Figures/RQ3.png}
  \caption{\label{fig:rq3}
           Overview of learning transfer result (from left to right): performance score organized by first and second exposure to each visualization technique, self-rated perceived learning transfer result on a scale of 1 to 7}
\end{figure}

\textbf{Analogy charts are effective independently, regardless of prior exposure to standard charts.} The result (Figure~\ref{fig:rq3}) from both participant groups suggested that participants performed similarly on analogy charts whether they had seen the standard charts before or not. The difference in average performance scores for participants first exposed to analogy charts (\textit{23.03, SD = 7.22}) versus those who viewed them after standard charts (\textit{22.78, SD = 7.44}) was insignificant (\(p = 0.929\)). This shows that analogy charts are independently practical learning tools.

Given that analogies are effective on their own, we examined how prior exposure to analogies influenced performance to understand the impact on learning transfer. The result indicates \textbf{visualization analogies promote learning transfer to standard charts.} Participants who saw analogy charts before standard charts performed significantly better on the standard charts. The average performance score for standard charts after analogy exposure was \textit{21.42 (SD = 6.73)}, compared to \textit{18.11 (SD = 6.19)} for those who saw standard charts first. This improvement was statistically significant \textit{(p = 0.007)}. 

Aligning with the performance score, \textbf{Participants reported high levels of perceived learning transfer from analogy to standard charts.} Specifically, \textit{76.56\%} reported that analogies made it easier to interpret the standard chart. Additionally, \textit{81.25\%} appreciated that analogies helped them understand key contexts of the standard chart, and \textit{81.25\%} felt analogies helped them recognize data relationships more clearly.


\subsection{RQ3 [Trade-Offs]: Balancing Data Encoding and User Attention}

\textbf{Visualization analogies do not introduce trade-offs in users' attention to data encoding.} Participants' descriptions of the analogy charts were as accurate as those of the standard charts. Without the chart title or dataset context, they identified the key idea of the charts using both visualization techniques. The mean description scores for the analogy \textit{(M = 9.01)} and baseline \textit{(M = 8.36)} were similar. A pairwise t-test showed no significant difference between the two techniques \textit{(p = 0.872)}.

We further examined the results in chart complexity dimension. \textbf{Visualization analogies significantly enhance interpretation accuracy for complex charts compared to standard charts.} Participants scored higher using visualization analogies \textit{M = 8.51, SD = 3.05)} than standard charts \textit{(M = 7.16, SD = 2.95)}when describing charts with harder interpretability. This difference was statistically significant \textit{(p = 0.047)}. Participants seemed to benefit from the additional visual cues provided by the analogies when interpreting more challenging charts. In contrast, the average scores for simple charts were similar between analogy \textit{(M =9.56, SD = 1.79)} and baseline \textit{M = 9.56, SD = 1.79)}. The pairwise t-test showed no significant difference \textit{(p = 0.087)}. This suggests that both techniques were equally effective in conveying the key information for simpler charts.


\subsection{RQ4 [Generalizability]: Effectiveness Across Diverse Learning Preferences}

\textbf{Visualization analogies are generalizable teaching techniques as they are adequate across different learning preferences.} An ANOVA F-test revealed no significant difference in performance scores among the VARK learning preference categories when using analogy charts \textit{(p = 0.826)}. The mean performance scores were similar across all groups: Auditory learners had a mean score of \textit{22.63 (SD = 7.27)}, Kinesthetic learners scored \textit{21.87 (SD = 7.08)}, Reading/Writing learners had \textit{20.16 (SD = 7.06)}, and Visual learners scored \textit{20.72 (SD = 7.12)}. 

\begin{figure}[htb]
  \centering
  \includegraphics[width=1\linewidth]{Figures/RQ5.png}
  \caption{\label{fig:rq5}
           (left) Performance score with analogies across all learning preferences. (right) Comparative preference result, each bar displays the percentages of participants favoring analogy or baseline for each of the displayed questions.}
\end{figure}

\subsection{RQ5 [User Preference]: Engagement and Comprehension Preferences for Visualization Analogies}

\textbf{Visualization analogies are perceived as more engaging.} Among all participants, a significant majority (\textit{83.59\%}) found visualization analogies more engaging than standard visualizations. One participant described the experience as \textit{"it feels like playing a game,"} suggesting that analogies' interactive and visually stimulating nature resonates broadly across different learning styles.

\textbf{Visualization analogies enhance cognitive processing and comprehension.} \textit{70.31\%} of participants reported that analogies required less mental effort to interpret, with comments like \textit{"the visuals look more realistic for me to interpret"} indicating that analogies streamline complex information processing and reduce cognitive load. Moreover, \textit{70.31\%} of participants appreciated analogies for their intuitiveness, stating that \textit{"visually, it makes clear everything you need to know and is easier to identify."} Additionally, \textit{63.28\%} of participants noted that analogies aided in recognizing patterns within the data more effectively. These observations suggest that analogies can effectively bridge the gap between complex data and the user's interpretation of underlying data structures by utilizing intuitive design elements.




==> egbibsample <==
@String{cgforum = "Computer Graphics Forum"}
@String{tog = "ACM TOG"}

@article{bach2023challenges,
  title={Challenges and opportunities in data visualization education: A call to action},
  author={Bach, Benjamin and Keck, Mandy and Rajabiyazdi, Fateme and Losev, Tatiana and Meirelles, Isabel and Dykes, Jason and Laramee, Robert S and AlKadi, Mashael and Stoiber, Christina and Huron, Samuel},
  journal={IEEE Transactions on Visualization \& Computer Graphics},
  publisher={IEEE},
  year={2023},
  doi={10.1109/TVCG.2023.3327378}
}

@inproceedings{huron2014constructive,
  title={Constructive visualization},
  author={Huron, Samuel and Carpendale, Sheelagh and Thudt, Alice and Tang, Anthony and Mauerer, Michael},
  booktitle={Proceedings of the 2014 conference on Designing interactive systems},
  pages={433--442},
  year={2014}
}

@article{perin2021students,
  title={What students learn with personal data physicalization},
  author={Perin, Charles},
  journal={IEEE Computer Graphics and Applications},
  volume={41},
  number={6},
  year={2021},
  publisher={IEEE}
}


@inproceedings{nobre2024reading,
  title={Reading Between the Pixels: Investigating the Barriers to Visualization Literacy},
  author={Nobre, Carolina and Zhu, Kehang and M{\"o}rth, Eric and Pfister, Hanspeter and Beyer, Johanna},
  booktitle={Proceedings of the CHI Conference on Human Factors in Computing Systems},
  pages={1--17},
  year={2024},
  doi = {10.1145/3613904.3642760},
}

@article{chang2024strategies,
  title={Strategies and difficulties during students’ construction of data visualizations},
  author={Chang, Hsin-Yi and Chang, Yen-Jung and Tsai, Meng-Jung},
  journal={International Journal of STEM Education},
  volume={11},
  number={1},
  pages={11},
  year={2024},
  publisher={Springer}
}


@inproceedings{analogies,
booktitle = {EuroVis 2025 - Education Papers},
editor = {Aurisano, Jillian and Laramee, Robert S. and Nobre, Carolina},
title = {{From Reality to Recognition: Evaluating Visualization Analogies for Novice Chart Comprehension}},
author = {Huang, Oliver and Lee, Patrick Yung Kang and Nobre, Carolina},
year = {2025},
publisher = {The Eurographics Association},
ISBN = {978-3-03868-273-8},
DOI = {10.2312/eved.20251004}
}
        


@article{grammel2010information,
  title={How information visualization novices construct visualizations},
  author={Grammel, Lars and Tory, Melanie and Storey, Margaret-Anne},
  journal={IEEE transactions on Visualization \& Computer Graphics},
  volume={16},
  number={6},
  year={2010},
}

@article{choe2024enhancing,
  title={Enhancing Data Literacy On-demand: LLMs as Guides for Novices in Chart Interpretation},
  author={Choe, Kiroong and Lee, Chaerin and Lee, Soohyun and Song, Jiwon and Cho, Aeri and Kim, Nam Wook and Seo, Jinwook},
  journal={IEEE Transactions on Visualization and Computer Graphics},
  year={2024},
  publisher={IEEE}
}

@article{harrison2006teaching,
  title={Teaching and learning with analogies: Friend or foe?},
  author={Harrison, Allan G and Treagust, David F},
  journal={Metaphor and analogy in science education},
  pages={11--24},
  doi = {10.1007/1-4020-3830-5_2},
  year={2006},
  publisher={Springer}
}

@inproceedings{cao2016examining,
  title={Examining the value of analogies in introductory computing},
  author={Cao, Yingjun and Porter, Leo and Zingaro, Daniel},
  booktitle={Proceedings of ACM Conference on International computing education research},
  year={2016}
}

@inproceedings{harsley2016incorporating,
  title={Incorporating analogies and worked out examples as pedagogical strategies in a computer science tutoring system},
  author={Harsley, Rachel and Green, Nick and Alizadeh, Mehrdad and Acharya, Sabita and Fossati, Davide and Di Eugenio, Barbara and AlZoubi, Omar},
  booktitle={Proceedings of the 47th acm technical symposium on computing science education},
  pages={675--680},
  year={2016}
}

@inproceedings{saxena2021analogy,
  title={Analogy-based Instruction for Effective Teaching of Abstract Concepts in Computer Science},
  author={Saxena, Pawan and Singh, Sanjay and Gupta, Gopal},
  booktitle={7th International Conference on Higher Education Advances (HEAd'21)},
  pages={377--385},
  year={2021},
  organization={Editorial Universitat Polit{\`e}cnica de Val{\`e}ncia}
}a


@article{nuamah_evaluating_2020,
	title = {Evaluating effectiveness of information visualizations using cognitive fit theory: A neuroergonomics approach},
	volume = {88},
	issn = {0003-6870},
	doi = {10.1016/j.apergo.2020.103173},
	pages = {103173},
	journaltitle = {Applied Ergonomics},
	author = {Nuamah, Joseph K. and Seong, Younho and Jiang, Steven and Park, Eui and Mountjoy, Daniel},
	date = {2020-10-01},
}


@article{locoro_visual_2021,
author = {Locoro, Angela and Fisher, Jr, William and Mari, Luca},
year = {2021},
month = {05},
title = {Visual Information Literacy: Definition, Construct Modeling and Assessment},
journal = {IEEE Access},
doi = {10.1109/ACCESS.2021.3078429}
}


@article{sarker_data_2021,
	title = {Data Science and Analytics: An Overview from Data-Driven Smart Computing, Decision-Making and Applications Perspective},
	volume = {2},
	issn = {2662-995X},
	doi = {10.1007/s42979-021-00765-8},
	pages = {377},
	number = {5},
	journaltitle = {Sn Computer Science},
	shortjournal = {{SN} Comput Sci},
	author = {Sarker, Iqbal H.},
	date = {2021},
}

@ARTICLE{borkin_what_2013,
  author={Borkin, Michelle A. and Vo, Azalea A. and Bylinskii, Zoya and Isola, Phillip and Sunkavalli, Shashank and Oliva, Aude and Pfister, Hanspeter},
  journal={IEEE Transactions on Visualization and Computer Graphics}, 
  title={What Makes a Visualization Memorable?}, 
  year={2013},
  volume={19},
  number={12},
  doi={10.1109/TVCG.2013.234}}


@article{https://doi.org/10.1111/cgf.14031,
    author = {Hogräfer, Marius and Heitzler, Magnus and Schulz, Hans-Jörg},
    title = {The State of the Art in Map-Like Visualization},
    journal = {Computer Graphics Forum},
    volume = {39},
    number = {3},
    pages = {647-674},
    doi = {https://doi.org/10.1111/cgf.14031},
    year = {2020}
}


@article{DVLD,
    author = {Borner, Katy and Bueckle, Andreas and Ginda, Michael},
    year = {2019},
    title = {Data visualization literacy: Definitions, conceptual frameworks, exercises, and assessments},
    volume = {116},
    journal = {Proceedings of the National Academy of Sciences},
    doi = {10.1073/pnas.1807180116}
}


@inproceedings{kim_generating_2016,
	title = {Generating Personalized Spatial Analogies for Distances and Areas},
	doi = {10.1145/2858036.2858440},
	pages = {38--48},
	booktitle = {Proceedings of {CHI} Conference on Human Factors in Computing Systems},
	publisher = {Association for Computing Machinery},
	author = {Kim, Yea-Seul and Hullman, Jessica and Agrawala, Maneesh},
	year = {2016},
}


@article{lin_effectiveness_1996,
	title = {The effectiveness of teaching science with pictorial analogies},
	volume = {26},
	issn = {1573-1898},
	doi = {10.1007/BF02357457},
	pages = {495--511},
	number = {4},
	journal = {Research in Science Education},
	author = {Lin, Huann-shyang and Shiau, Bih-ruh and Lawrenz, Frances},
	year = {1996},
}



@book{marzano_classroom_2001,
	title = {Classroom Instruction That Works: Research-Based Strategies for Increasing Student Achievement},
	isbn = {978-0-87120-504-9},
	publisher = {Association for Supervision and Curriculum Development},
	author = {Marzano, Robert J. and Pickering, Debra J. and Pollock, Jane E.},
	year = {2001}
}



@article{reading_turchioe_visual_2020,
author = {Turchioe, Meghan and Grossman, Lisa and Myers, Annie and Baik, Dawon and Goyal, Parag and Masterson Creber, Ruth},
year = {2020},
month = {01},
title = {Visual analogies, not graphs, increase patients' comprehension of changes in their health status},
volume = {27},
journal = {Journal of the American Medical Informatics Association},
doi = {10.1093/jamia/ocz217}
}

@inproceedings{chen_beyond_2024,
	location = {Honolulu {HI} {USA}},
	title = {Beyond Numbers: Creating Analogies to Enhance Data Comprehension and Communication with Generative {AI}},
	isbn = {9798400703300},
	doi = {10.1145/3613904.3642480},
	booktitle = {Proceedings of {CHI} Conference on Human Factors in Computing Systems},
	author = {Chen, Qing and Shuai, Wei and Zhang, Jiyao and Sun, Zhida and Cao, Nan},
	year = {2024},
        month = {5}
}

@inproceedings{lopes_teaching_2024,
	title = {Teaching Information Visualization through Situated Design: Case Studies from the Classroom},
	doi = {10.1109/EduVIS63909.2024.00010},
	eventtitle = {2024 {IEEE} {VIS} Workshop on Visualization Education, Literacy, and Activities ({EduVIS})},
	pages = {38--43},
	booktitle = {2024 {IEEE} {VIS} Workshop on Visualization Education, Literacy, and Activities ({EduVIS})},
	author = {Lopes, Renata and Reznik, Regina and Kosminsky, Doris},
	date = {2024-10},
}

@article{morrill_breaking_2017,
	title = {Breaking the bar chart: why chart types are holding us back and how metaphors can help.},
	shorttitle = {Breaking the bar chart},
	author = {Morrill, Ryan},
	year = {2017},
        journal = {Northeastern University},
	doi = {10.17760/D20257369},
}

@inproceedings{riederer_put_2018,
	location = {New York, {NY}, {USA}},
	title = {To Put That in Perspective: Generating Analogies that Make Numbers Easier to Understand},
	isbn = {978-1-4503-5620-6},
	doi = {10.1145/3173574.3174122},
	shorttitle = {To Put That in Perspective},
	pages = {1--10},
	booktitle = {Proceedings of {CHI} Conference on Human Factors in Computing Systems},
	author = {Riederer, Christopher and Hofman, Jake M. and Goldstein, Daniel G.},
	year = {2018}
}

@inproceedings{hullman_improving_2018,
	title = {Improving Comprehension of Measurements Using Concrete Re-expression Strategies},
	doi = {10.1145/3173574.3173608},
	pages = {1--12},
	booktitle = {Proceedings of {CHI} Conference on Human Factors in Computing Systems},
	author = {Hullman, Jessica and Kim, Yea-Seul and Nguyen, Francis and Speers, Lauren and Agrawala, Maneesh},
	year = {2018},
}

@article{chevalier_using_2013,
	title = {Using Concrete Scales: A Practical Framework for Effective Visual Depiction of Complex Measures},
	volume = {19},
	issn = {1077-2626},
	doi = {10.1109/TVCG.2013.210},
	pages = {2426--2435},
	number = {12},
	journaltitle = {{IEEE} Transactions on Visualization and Computer Graphics},
	author = {Chevalier, Fanny and Vuillemot, Romain and Gali, Guia},
	date = {2013-12-01},
}


@article{spezzini_effects_nodate,
    author = {Spezzini, Susan},
    year = {2010},
    month = {07},
    title = {Effects of Visual Analogies on Learner Outcomes: Bridging from the Known to the Unknown},
    volume = {4},
    journal = {International Journal for the Scholarship of Teaching and Learning},
    doi = {10.20429/ijsotl.2010.040211}
}


@misc{bae_cultivating_2022,
	title = {Cultivating Visualization Literacy for Children Through Curiosity and Play},
	doi = {10.48550/arXiv.2208.05015},
	number = {{arXiv}:2208.05015},
	publisher = {{arXiv}},
	author = {Bae, S. Sandra and Vanukuru, Rishi and Yang, Ruhan and Gyory, Peter and Zhou, Ran and Do, Ellen Yi-Luen and Szafir, Danielle Albers},
	date = {2022-08-09},
	
}

@ARTICLE{huynh_designing_2020,
author={Huynh, Elaine and Nyhout, Angela and Ganea, Patricia and Chevalier, Fanny},
journal={ IEEE Transactions on Visualization \& Computer Graphics },
title={{ Designing Narrative-Focused Role-Playing Games for Visualization Literacy in Young Children }},
year={2021},
volume={27},
number={02},
doi={10.1109/TVCG.2020.3030464},
month=feb}


@article{chang_strategies_2024,
author = {Chang, Hsin-Yi and Chang, Yen-Jung and Tsai, Meng-Jung},
year = {2024},
month = {02},
title = {Strategies and difficulties during students’ construction of data visualizations},
journal = {International Journal of STEM Education},
doi = {10.1186/s40594-024-00463-w}
}

@article{ruchikachorn_learning_2015,
  author={Ruchikachorn, Puripant and Mueller, Klaus},
  journal={IEEE Transactions on Visualization and Computer Graphics}, 
  title={Learning Visualizations by Analogy: Promoting Visual Literacy through Visualization Morphing}, 
  year={2015},
  volume={21},
  doi={10.1109/TVCG.2015.2413786}
}

@article{chevalier_observations_nodate,
	title = {Observations and Reflections on Visualization Literacy in Elementary School},
	doi = {10.1109/MCG.2018.032421650},
        journal = {IEEE Computer Graphics \& Applications},
	author = {Chevalier, Fanny and Riche, Nathalie Henry and Alper, Basak and Plaisant, Catherine and Boy, Jeremy and Elmqvist, Niklas},
        year = {2018}
}

@article{lee_how_2016,
	title = {How do People Make Sense of Unfamiliar Visualizations?: A Grounded Model of Novice's Information Visualization Sensemaking},
	volume = {22},
	issn = {1941-0506},
	doi = {10.1109/TVCG.2015.2467195},
	pages = {499--508},
	number = {1},
	journaltitle = {{IEEE} Transactions on Visualization and Computer Graphics},
	author = {Lee, Sukwon and Kim, Sung-Hee and Hung, Ya-Hsin and Lam, Heidi and Kang, Youn-Ah and Yi, Ji Soo},
	date = {2016-01},
}

@inproceedings{lopes_teaching_2024,
	title = {Teaching Information Visualization through Situated Design: Case Studies from the Classroom},
	doi = {10.1109/EduVIS63909.2024.00010},
	shorttitle = {Teaching Information Visualization through Situated Design},
	eventtitle = {2024 {IEEE} {VIS} Workshop on Visualization Education, Literacy, and Activities ({EduVIS})},
	pages = {38--43},
	booktitle = {2024 {IEEE} {VIS} Workshop on Visualization Education, Literacy, and Activities ({EduVIS})},
	author = {Lopes, Renata and Reznik, Regina and Kosminsky, Doris},
	date = {2024-10},
}

@article{fuchs_treeducation_2024,
	title = {{TreEducation}: A Visual Education Platform for Teaching Treemap Layout Algorithms},
	volume = {{PP}},
	issn = {1941-0506},
	doi = {10.1109/TVCG.2024.3393012},
	journaltitle = {{IEEE} transactions on visualization and computer graphics},
	author = {Fuchs, Johannes and Jackl, Bastian and Juttler, Michael and Keim, Daniel A. and Sevastjanova, Rita},
	date = {2024-04-24},
}

@book{firat_constructivism-based_2023,
	title = {A Constructivism-based Approach to Treemap Literacy in the Classroom},
	isbn = {978-3-03868-210-3},
	publisher = {The Eurographics Association},
	author = {Firat, Elif E. and Lang, Colm and Srinivas, Bhumika and Peng, Ilena and Laramee, Robert S. and Joshi, Alark},
	date = {2023},
	doi = {10.2312/eged.20231016}
}

@article{adar_roboviz_2022,
author={Adar, Eytan and Lee-Robbins, Elsie},
journal={ IEEE Transactions on Visualization \& Computer Graphics },
title={{ Roboviz: A Game-Centered Project for Information Visualization Education }},
year={2023},
doi={10.1109/TVCG.2022.3209402},
publisher={IEEE Computer Society},
address={Los Alamitos, CA, USA},
month=jan
}

@article{aunhabundit_visualizing_2024,
title={Visualizing Success: Amplifying Learning Outcomes across VARK Learning Preferences through Visual Notes}, volume={2024}, number={6}, journal={Science, Technology, and Social Sciences Procedia}, author={Aunhabundit, Nattapon and Cheng Chieh Lu, Allan}, year={2024}, month={Jul.}, pages={ICCM03} }


@article{VARKGuide,
  title={Understanding your student: using the VARK model.},
  author={Ivan James Prithishkumar and S A Michael},
  journal={Journal of postgraduate medicine},
  year={2014},
  doi = {10.4103/0022-3859.132337}
}



@article{aisami_learning_2015,
	title = {Learning Styles and Visual Literacy for Learning and Performance},
	volume = {176},
	issn = {1877-0428},
	doi = {10.1016/j.sbspro.2015.01.508},
	series = {International Educational Technology Conference, {IETC} 2014, 3-5 September 2014, Chicago, {IL}, {USA}},
	pages = {538--545},
	journaltitle = {Procedia - Social and Behavioral Sciences},
	author = {Aisami, Riad S.},
	date = {2015-02-20},
}



@inproceedings{tkachev_metaphorical_2022,
	title = {Metaphorical Visualization: Mapping Data to Familiar Concepts},
	isbn = {978-1-4503-9156-6},
	doi = {10.1145/3491101.3516393},
	pages = {1--10},
	booktitle = {{CHI} Conference on Human Factors in Computing Systems Extended Abstracts},
	publisher = {{ACM}},
	author = {Tkachev, Gleb and Cutura, Rene and Sedlmair, Michael and Frey, Steffen and Ertl, Thomas},
	date = {2022-04-27},
}

@inproceedings{lopes_teaching_2024,
	title = {Teaching Information Visualization through Situated Design: Case Studies from the Classroom},
	doi = {10.1109/EduVIS63909.2024.00010},
	eventtitle = {2024 {IEEE} {VIS} Workshop on Visualization Education, Literacy, and Activities ({EduVIS})},
	pages = {38--43},
	author = {Lopes, Renata and Reznik, Regina and Kosminsky, Doris},
	date = {2024-10},
}

@article{segel_narrative_2010,
	title = {Narrative Visualization: Telling Stories with Data},
	volume = {16},
	issn = {1077-2626},
	doi = {10.1109/TVCG.2010.179},
	pages = {1139--1148},
	journaltitle = {{IEEE} Transactions on Visualization and Computer Graphics},
	author = {Segel, E and Heer, J},
	date = {2010-11},
}


@article{lo_learning_2019,
	title = {Learning Vis Tools: Teaching Data Visualization Tutorials},
	doi = {10.48550/arXiv.1907.08796},
	publisher = {{arXiv}},
	author = {Lo, Leo Yu-Ho and Ming, Yao and Qu, Huamin},
	date = {2019-10-07},
}

@inproceedings{doukakis2007using,
  title={Using animated interactive analogies in teaching basic programming concepts and structures},
  author={Doukakis, Dimitrios and Tsaganou, Grammatiki and Grigoriadou, Maria},
  booktitle={Proceedings of the ACM Conference on the State of: Informatics Education Europe II, Thessaloniki, Greece},
  pages={257--265},
  year={2007}
}


@misc{bae_cultivating_2022,
	title = {Cultivating Visualization Literacy for Children Through Curiosity and Play},
	doi = {10.48550/arXiv.2208.05015},
	publisher = {{arXiv}},
	author = {Bae, S. Sandra and Vanukuru, Rishi and Yang, Ruhan and Gyory, Peter and Zhou, Ran and Do, Ellen Yi-Luen and Szafir, Danielle Albers},
	date = {2022-08-09},
}


@inproceedings{burns_who_2023,
	title = {Who Do We Mean When We Talk About Visualization Novices?},
	isbn = {978-1-4503-9421-5},
	doi = {10.1145/3544548.3581524},
	pages = {1--16},
	booktitle = {Proceedings of {CHI} Conference on Human Factors in Computing Systems},
	publisher = {Association for Computing Machinery},
	author = {Burns, Alyxander and Lee, Christiana and Chawla, Ria and Peck, Evan and Mahyar, Narges},
	year={2023},
}


@article{choe_enhancing_2024,
	title = {Enhancing Data Literacy On-demand: {LLMs} as Guides for Novices in Chart Interpretation},
	issn = {1941-0506},
	doi = {10.1109/TVCG.2024.3413195},
	pages = {1--17},
	journaltitle = {{IEEE} Transactions on Visualization and Computer Graphics},
	author = {Choe, Kiroong and Lee, Chaerin and Lee, Soohyun and Song, Jiwon and Cho, Aeri and Kim, Nam Wook and Seo, Jinwook},
	date = {2024},
}

@inproceedings{gabler_diagram_2019,
	title = {Diagram Safari: A Visualization Literacy Game for Young Children},
	doi = {10.1145/3341215.3356283},
	booktitle = {Extended Abstracts of the Annual Symposium on Computer-Human Interaction in Play Companion},
	author = {Gäbler, Johannes and Winkler, Christoph and Lengyel, Nóra and Aigner, Wolfgang and Stoiber, Christina and Wallner, Günter and Kriglstein, Simone},
	year = {2019}
}


@book{denis_spss_2018,
	title = {{SPSS} Data Analysis for Univariate, Bivariate, and Multivariate Statistics},
        doi = {DOI: 10.1002/9781119465775},
	publisher = {John Wiley \& Sons},
	author = {Denis, Daniel J.},
	year = {2018},
}


@inproceedings{strantz_data_2022,
	title = {Data as “Brickolage”: Teaching Material Data Visualization Design with {LEGO}},
	isbn = {978-1-4503-9246-4},
	doi = {10.1145/3513130.3558990},
	eventtitle = {{SIGDOC} '22: The 40th {ACM} International Conference on Design of Communication},
	pages = {130--135},
	booktitle = {The 40th {ACM} International Conference on Design of Communication},
	publisher = {{ACM}},
	author = {Strantz, Adam},
	date = {2022-10-06},
}


@inproceedings{andry_interpreting_2021,
	location = {Yokohama Japan},
	title = {Interpreting the Effect of Embellishment on Chart Visualizations},
	isbn = {978-1-4503-8096-6},
	doi = {10.1145/3411764.3445739},
	booktitle = {Proceedings of {CHI} Conference on Human Factors in Computing Systems},
	publisher = {{ACM}},
	author = {Andry, Tiffany and Hurter, Christophe and Lambotte, François and Fastrez, Pierre and Telea, Alexandru},
	year = {2021},
}

@inproceedings{bateman_useful_2010,
	title = {Useful junk?: the effects of visual embellishment on comprehension and memorability of charts},
	isbn = {978-1-60558-929-9},
	doi = {10.1145/1753326.1753716},
	booktitle = {Proceedings of {CHI} Conference on Human Factors in Computing Systems},
	publisher = {{ACM}},
	author = {Bateman, Scott and Mandryk, Regan L. and Gutwin, Carl and Genest, Aaron and {McDine}, David and Brooks, Christopher},
	year={2010},
}

@misc{chen_vizbelle_2022,
	title = {{VizBelle}: A Design Space of Embellishments for Data Visualization},
	doi = {10.48550/arXiv.2209.03642},
	shorttitle = {{VizBelle}},
	publisher = {{arXiv}},
	author = {Chen, Qing and Liu, Ziyan and Wang, Chengwei and Lan, Xingyu and Chen, Ying and Chen, Siming and Cao, Nan},
	date = {2022-09-08},
}


@article{walny_exploratory_2015,
	title = {An Exploratory Study of Data Sketching for Visual Representation},
	volume = {34},
	issn = {1467-8659},
	doi = {10.1111/cgf.12635},
	pages = {231--240},
	number = {3},
	journaltitle = {Computer Graphics Forum},
	author = {Walny, J. and Huron, S. and Carpendale, S.},
	date = {2015},
}


@article{choi_situated_1995,
	title = {Situated cognition and learning environments: Roles, structures, and implications for design},
	volume = {43},
	number = {2},
	journal = {Educational Technology Research and Development},
	author = {Choi, Jeong-Im and Hannafin, Michael},
	year = {1995},
}


@article{richer_scalability_2024,
author = {Richer, Ga\"{e}lle and Pister, Alexis and Abdelaal, Moataz and Fekete, Jean-Daniel and Sedlmair, Michael and Weiskopf, Daniel},
title = {Scalability in Visualization},
year = {2024},
issue_date = {July 2024},
publisher = {IEEE Educational Activities Department},
address = {USA},
volume = {30},
number = {7},
doi = {10.1109/TVCG.2022.3231230},
journal = {IEEE Transactions on Visualization and Computer Graphics},
month = jul
}

@conference{huron2020ieee,
    author = {Samuel Huron and Benjamin Bach and Georgia Panagiotidou and Mandy Keck and Roberts, Jonathan C. and Sheelagh Carpendale},
    booktitle = {The 2nd IEEE VIS Workshop} ,
    title = {Data Vis Activities to Facilitate Learning, Reflecting, Discussing and Designing},
    year = {2021}
}

















